Hierarchical Representations and Explicit Memory: Learning Effective Navigation Policies on 3D Scene Graphs using Graph Neural Networks

Representations are crucial for a robot to learn effective navigation policies. Recent work has shown that mid-level perceptual abstractions, such as depth estimates or 2D semantic segmentation, lead to more effective policies when provided as observations in place of raw sensor data (e.g., RGB images). However, such policies must still learn latent three-dimensional scene properties from mid-level abstractions. In contrast, high-level, hierarchical representations such as 3D scene graphs explicitly provide a scene's geometry, topology, and semantics, making them compelling representations for navigation. In this work, we present a reinforcement learning framework that leverages high-level hierarchical representations to learn navigation policies. Towards this goal, we propose a graph neural network architecture and show how to embed a 3D scene graph into an agent-centric feature space, which enables the robot to learn policies for low-level action in an end-to-end manner. For each node in the scene graph, our method uses features that capture occupancy and semantic content, while explicitly retaining memory of the robot trajectory. We demonstrate the effectiveness of our method against commonly used visuomotor policies in a challenging object search task. These experiments and supporting ablation studies show that our method leads to more effective object search behaviors, exhibits improved long-term memory, and successfully leverages hierarchical information to guide its navigation objectives.

==> includes/gnn_figure.tex <==

\resizebox{150pt}{125pt}{%
\begin{tikzpicture}[
greennode/.style={circle, draw=black, fill=black!30!green, line width=0.5mm, minimum size=10mm},
rednode/.style={circle, draw=black, fill=black!20!red, line width=0.5mm, minimum size=10mm},
orangenode/.style={circle, draw=black, fill=black!10!orange, line width=0.5mm, minimum size=10mm},
bluenode/.style={circle, draw=black, fill=black!20!blue, line width=0.5mm, minimum size=10mm},
]

% level 1 

\coordinate (l1) at (-5, 0);

\node[greennode] at ( $(l1) + (0, 0)$) (greennode1) {};
\node[rednode] at ( $(l1) + (1, 1.5)$) (rednode1) {};
\node[orangenode] at ( $(l1) + (1, -1.3)$) (orangenode1) {};
\node[bluenode] at ( $(l1) + (2, .5)$) (bluenode1) {};

\draw[very thick] (greennode1) -- (rednode1);
\draw[very thick] (greennode1) -- (orangenode1);
\draw[very thick] (greennode1) -- (bluenode1);
\draw[very thick] (rednode1) -- (bluenode1);

\draw[->, very thick] (-2, 0) -- (-1, 0);
\draw[->, very thick] (-2, -3) -- (-1.5, -4);
\draw[->, very thick] (-2, 3) -- (-1.5, 4);

% level 2

\coordinate (l2) at (0, 0);

\node[rednode] at ( $(l2) + (0, 0)$) (greennode2) {};
\node[greennode] at ( $(l2) + (1, 1.5)$) (rednode2) {};
\node[orangenode] at ( $(l2) + (1, -1.3)$) (orangenode2) {};
\node[bluenode] at ( $(l2) + (2, .5)$) (bluenode2) {};

\draw[very thick] (greennode2) -- (rednode2);
\draw[very thick] (greennode2) -- (orangenode2);
\draw[very thick] (greennode2) -- (bluenode2);
\draw[very thick] (rednode2) -- (bluenode2);

\coordinate (l21) at (0, 5);

\node[greennode] at ( $(l21) + (0, 0)$) (greennode21) {};
\node[orangenode] at ( $(l21) + (1, 1.5)$) (rednode21) {};
\node[bluenode] at ( $(l21) + (1, -1.3)$) (orangenode21) {};
\node[greennode] at ( $(l21) + (2, .5)$) (bluenode21) {};

\draw[very thick] (greennode21) -- (rednode21);
\draw[very thick] (greennode21) -- (orangenode21);
\draw[very thick] (greennode21) -- (bluenode21);
\draw[very thick] (rednode21) -- (bluenode21);

\node[font=\Huge] at (1, 2.5) {$\vdots$};

\coordinate (l22) at (0, -5);

\node[greennode] at ( $(l22) + (0, 0)$) (greennode21) {};
\node[rednode] at ( $(l22) + (1, 1.5)$) (rednode21) {};
\node[bluenode] at ( $(l22) + (1, -1.3)$) (orangenode21) {};
\node[orangenode] at ( $(l22) + (2, .5)$) (bluenode21) {};

\draw[very thick] (greennode21) -- (rednode21);
\draw[very thick] (greennode21) -- (orangenode21);
\draw[very thick] (greennode21) -- (bluenode21);
\draw[very thick] (rednode21) -- (bluenode21);

\node[font=\Huge] at (1, -2.5) {$\vdots$};


\coordinate (l22) at (5, 0);

\node[greennode] at ( $(l22) + (0, 0)$) (greennode21) {};
\node[rednode] at ( $(l22) + (1, 1.5)$) (rednode21) {};
\node[bluenode] at ( $(l22) + (1, -1.3)$) (orangenode21) {};
\node[orangenode] at ( $(l22) + (2, .5)$) (bluenode21) {};

\draw[very thick] (greennode21) -- (rednode21);
\draw[very thick] (greennode21) -- (orangenode21);
\draw[very thick] (greennode21) -- (bluenode21);
\draw[very thick] (rednode21) -- (bluenode21);

\draw[->, very thick] (3, 0) -- (4, 0);
\draw[->, very thick] (3, 5) -- (4, 5);
\draw[->, very thick] (3, -5) -- (4, -5);


\coordinate (l22) at (5, 5);

\node[orangenode] at ( $(l22) + (0, 0)$) (greennode21) {};
\node[bluenode] at ( $(l22) + (1, 1.5)$) (rednode21) {};
\node[greennode] at ( $(l22) + (1, -1.3)$) (orangenode21) {};
\node[rednode] at ( $(l22) + (2, .5)$) (bluenode21) {};

\draw[very thick] (greennode21) -- (rednode21);
\draw[very thick] (greennode21) -- (orangenode21);
\draw[very thick] (greennode21) -- (bluenode21);
\draw[very thick] (rednode21) -- (bluenode21);

\node[font=\Huge] at (6, 2.5) {$\vdots$};


\coordinate (l22) at (5, -5);

\node[greennode] at ( $(l22) + (0, 0)$) (greennode21) {};
\node[bluenode] at ( $(l22) + (1, 1.5)$) (rednode21) {};
\node[orangenode] at ( $(l22) + (1, -1.3)$) (orangenode21) {};
\node[rednode] at ( $(l22) + (2, .5)$) (bluenode21) {};

\draw[very thick] (greennode21) -- (rednode21);
\draw[very thick] (greennode21) -- (orangenode21);
\draw[very thick] (greennode21) -- (bluenode21);
\draw[very thick] (rednode21) -- (bluenode21);

\node[font=\Huge] at (6, -2.5) {$\vdots$};


\coordinate (l22) at (10, 0);

\node[greennode] at ( $(l22) + (0, 0)$) (greennode21) {};
\node[rednode] at ( $(l22) + (1, 1.5)$) (rednode21) {};
\node[orangenode] at ( $(l22) + (1, -1.3)$) (orangenode21) {};
\node[bluenode] at ( $(l22) + (2, .5)$) (bluenode21) {};

\draw[very thick] (greennode21) -- (rednode21);
\draw[very thick] (greennode21) -- (orangenode21);
\draw[very thick] (greennode21) -- (bluenode21);
\draw[very thick] (rednode21) -- (bluenode21);

\draw[->, very thick] (8, 0) -- (9, 0);

% \draw[->, very thick] (-2, 0) -- (-1, 0);
\draw[->, very thick] (8.5, -4) -- (9, -3);
\draw[->, very thick] (8.5, 4) -- (9, 3);


% \draw[->, very thick] (13, 0) -- (14, 0)

\end{tikzpicture}
}


==> includes/gnn_figure_v2.tex <==

% \resizebox{150pt}{125pt}{%
\begin{tikzpicture}[
greennode/.style={circle, draw=black, fill=black!30!green, line width=0.5mm, minimum size=8mm},
rednode/.style={circle, draw=black, fill=black!20!red, line width=0.5mm, minimum size=8mm},
orangenode/.style={circle, draw=black, fill=black!10!orange, line width=0.5mm, minimum size=8mm},
bluenode/.style={circle, draw=black, fill=black!20!blue, line width=0.5mm, minimum size=8mm},
]

% level 1 
\coordinate (base1) at (-5, 0);

\coordinate (l11) at (base1);
\node[greennode] at ( $(l11) + (0, 0)$) (greennode1) {};
\node[greennode] at ( $(l11) + (-1.5, -1)$) (greennode2) {};
\node[rednode] at ( $(l11) + (1, 1.5)$) (rednode1) {};
\node[rednode] at ( $(l11) + (-0.75, 1.75)$) (rednode2) {};
\node[orangenode] at ( $(l11) + (1, -1.3)$) (orangenode1) {};
\node[bluenode] at ( $(l11) + (2, .5)$) (bluenode1) {};
\node[bluenode] at ( $(l11) + (2.75, -0.6)$) (bluenode2) {};
\node[bluenode] at ( $(l11) + (3.25, 1.75)$) (bluenode3) {};
\draw[very thick] (greennode2) -- (orangenode1);
\draw[very thick] (greennode2) -- (rednode2);
\draw[very thick] (rednode1) -- (rednode2);
\draw[very thick] (rednode2) -- (greennode1);
\draw[very thick] (greennode1) -- (greennode2);
\draw[very thick] (greennode1) -- (orangenode1);
\draw[very thick] (greennode1) -- (bluenode1);
\draw[very thick] (rednode1) -- (bluenode1);
\draw[very thick] (bluenode1) -- (bluenode2);
\draw[very thick] (bluenode1) -- (bluenode3);
\draw[very thick] (orangenode1) -- (bluenode1);

\draw[->, line width=2mm] (-0.7, 0) -- (0.3, 0);
\draw[->, line width=2mm] (-0.7, 2.5) -- (0.3, 3.25);
\draw[->, line width=2mm] (-0.7, -2.5) -- (0.3, -3.25);



% ------------- second level -------------------
\coordinate (base2) at ($(base1) + (8, 0)$);

\coordinate (l11) at (base2);
\node[greennode] at ( $(l11) + (0, 0)$) (greennode1) {};
\node[rednode] at ( $(l11) + (-1.5, -1)$) (greennode2) {};
\node[rednode] at ( $(l11) + (1, 1.5)$) (rednode1) {};
\node[greennode] at ( $(l11) + (-0.75, 1.75)$) (rednode2) {};
\node[orangenode] at ( $(l11) + (1, -1.3)$) (orangenode1) {};
\node[orangenode] at ( $(l11) + (2, .5)$) (bluenode1) {};
\node[bluenode] at ( $(l11) + (2.75, -0.6)$) (bluenode2) {};
\node[bluenode] at ( $(l11) + (3.25, 1.75)$) (bluenode3) {};
\draw[very thick] (greennode2) -- (orangenode1);
\draw[very thick] (greennode2) -- (rednode2);
\draw[very thick] (rednode1) -- (rednode2);
\draw[very thick] (rednode2) -- (greennode1);
\draw[very thick] (greennode1) -- (greennode2);
\draw[very thick] (greennode1) -- (orangenode1);
\draw[very thick] (greennode1) -- (bluenode1);
\draw[very thick] (rednode1) -- (bluenode1);
\draw[very thick] (bluenode1) -- (bluenode2);
\draw[very thick] (bluenode1) -- (bluenode3);
\draw[very thick] (orangenode1) -- (bluenode1);

\coordinate (l11) at ($(base2) + (0, -6.5)$);
\node[rednode] at ( $(l11) + (0, 0)$) (greennode1) {};
\node[greennode] at ( $(l11) + (-1.5, -1)$) (greennode2) {};
\node[rednode] at ( $(l11) + (1, 1.5)$) (rednode1) {};
\node[rednode] at ( $(l11) + (-0.75, 1.75)$) (rednode2) {};
\node[bluenode] at ( $(l11) + (1, -1.3)$) (orangenode1) {};
\node[bluenode] at ( $(l11) + (2, .5)$) (bluenode1) {};
\node[bluenode] at ( $(l11) + (2.75, -0.6)$) (bluenode2) {};
\node[bluenode] at ( $(l11) + (3.25, 1.75)$) (bluenode3) {};
\draw[very thick] (greennode2) -- (orangenode1);
\draw[very thick] (greennode2) -- (rednode2);
\draw[very thick] (rednode1) -- (rednode2);
\draw[very thick] (rednode2) -- (greennode1);
\draw[very thick] (greennode1) -- (greennode2);
\draw[very thick] (greennode1) -- (orangenode1);
\draw[very thick] (greennode1) -- (bluenode1);
\draw[very thick] (rednode1) -- (bluenode1);
\draw[very thick] (bluenode1) -- (bluenode2);
\draw[very thick] (bluenode1) -- (bluenode3);
\draw[very thick] (orangenode1) -- (bluenode1);

\coordinate (l11) at ($(base2) + (0, 6.5)$);
\node[greennode] at ( $(l11) + (0, 0)$) (greennode1) {};
\node[greennode] at ( $(l11) + (-1.5, -1)$) (greennode2) {};
\node[rednode] at ( $(l11) + (1, 1.5)$) (rednode1) {};
\node[rednode] at ( $(l11) + (-0.75, 1.75)$) (rednode2) {};
\node[orangenode] at ( $(l11) + (1, -1.3)$) (orangenode1) {};
\node[bluenode] at ( $(l11) + (2, .5)$) (bluenode1) {};
\node[bluenode] at ( $(l11) + (2.75, -0.6)$) (bluenode2) {};
\node[bluenode] at ( $(l11) + (3.25, 1.75)$) (bluenode3) {};
\draw[very thick] (greennode2) -- (orangenode1);
\draw[very thick] (greennode2) -- (rednode2);
\draw[very thick] (rednode1) -- (rednode2);
\draw[very thick] (rednode2) -- (greennode1);
\draw[very thick] (greennode1) -- (greennode2);
\draw[very thick] (greennode1) -- (orangenode1);
\draw[very thick] (greennode1) -- (bluenode1);
\draw[very thick] (rednode1) -- (bluenode1);
\draw[very thick] (bluenode1) -- (bluenode2);
\draw[very thick] (bluenode1) -- (bluenode3);
\draw[very thick] (orangenode1) -- (bluenode1);

\draw[->, line width=2mm] (7.5, 0) -- (8.5, 0);
\draw[->, line width=2mm] (7.5, -6.5) -- (8.5, -6.5);
\draw[->, line width=2mm] (7.5, 6.5) -- (8.5, 6.5);


% ------------- third level -------------------
\coordinate (base2) at ($(base1) + (16, 0)$);

\coordinate (l11) at (base2);
\node[rednode] at ( $(l11) + (0, 0)$) (greennode1) {};
\node[greennode] at ( $(l11) + (-1.5, -1)$) (greennode2) {};
\node[rednode] at ( $(l11) + (1, 1.5)$) (rednode1) {};
\node[rednode] at ( $(l11) + (-0.75, 1.75)$) (rednode2) {};
\node[rednode] at ( $(l11) + (1, -1.3)$) (orangenode1) {};
\node[bluenode] at ( $(l11) + (2, .5)$) (bluenode1) {};
\node[bluenode] at ( $(l11) + (2.75, -0.6)$) (bluenode2) {};
\node[orangenode] at ( $(l11) + (3.25, 1.75)$) (bluenode3) {};
\draw[very thick] (greennode2) -- (orangenode1);
\draw[very thick] (greennode2) -- (rednode2);
\draw[very thick] (rednode1) -- (rednode2);
\draw[very thick] (rednode2) -- (greennode1);
\draw[very thick] (greennode1) -- (greennode2);
\draw[very thick] (greennode1) -- (orangenode1);
\draw[very thick] (greennode1) -- (bluenode1);
\draw[very thick] (rednode1) -- (bluenode1);
\draw[very thick] (bluenode1) -- (bluenode2);
\draw[very thick] (bluenode1) -- (bluenode3);
\draw[very thick] (orangenode1) -- (bluenode1);

\coordinate (l11) at ($(base2) + (0, -6.5)$);
\node[greennode] at ( $(l11) + (0, 0)$) (greennode1) {};
\node[greennode] at ( $(l11) + (-1.5, -1)$) (greennode2) {};
\node[rednode] at ( $(l11) + (1, 1.5)$) (rednode1) {};
\node[rednode] at ( $(l11) + (-0.75, 1.75)$) (rednode2) {};
\node[orangenode] at ( $(l11) + (1, -1.3)$) (orangenode1) {};
\node[bluenode] at ( $(l11) + (2, .5)$) (bluenode1) {};
\node[bluenode] at ( $(l11) + (2.75, -0.6)$) (bluenode2) {};
\node[bluenode] at ( $(l11) + (3.25, 1.75)$) (bluenode3) {};
\draw[very thick] (greennode2) -- (orangenode1);
\draw[very thick] (greennode2) -- (rednode2);
\draw[very thick] (rednode1) -- (rednode2);
\draw[very thick] (rednode2) -- (greennode1);
\draw[very thick] (greennode1) -- (greennode2);
\draw[very thick] (greennode1) -- (orangenode1);
\draw[very thick] (greennode1) -- (bluenode1);
\draw[very thick] (rednode1) -- (bluenode1);
\draw[very thick] (bluenode1) -- (bluenode2);
\draw[very thick] (bluenode1) -- (bluenode3);
\draw[very thick] (orangenode1) -- (bluenode1);

\coordinate (l11) at ($(base2) + (0, 6.5)$);
\node[greennode] at ( $(l11) + (0, 0)$) (greennode1) {};
\node[greennode] at ( $(l11) + (-1.5, -1)$) (greennode2) {};
\node[rednode] at ( $(l11) + (1, 1.5)$) (rednode1) {};
\node[rednode] at ( $(l11) + (-0.75, 1.75)$) (rednode2) {};
\node[orangenode] at ( $(l11) + (1, -1.3)$) (orangenode1) {};
\node[bluenode] at ( $(l11) + (2, .5)$) (bluenode1) {};
\node[bluenode] at ( $(l11) + (2.75, -0.6)$) (bluenode2) {};
\node[bluenode] at ( $(l11) + (3.25, 1.75)$) (bluenode3) {};
\draw[very thick] (greennode2) -- (orangenode1);
\draw[very thick] (greennode2) -- (rednode2);
\draw[very thick] (rednode1) -- (rednode2);
\draw[very thick] (rednode2) -- (greennode1);
\draw[very thick] (greennode1) -- (greennode2);
\draw[very thick] (greennode1) -- (orangenode1);
\draw[very thick] (greennode1) -- (bluenode1);
\draw[very thick] (rednode1) -- (bluenode1);
\draw[very thick] (bluenode1) -- (bluenode2);
\draw[very thick] (bluenode1) -- (bluenode3);
\draw[very thick] (orangenode1) -- (bluenode1);

\draw[->, line width=2mm] (15.5, 0) -- (16.5, 0);
\draw[->, line width=2mm] (15.5, 3.25) -- (16.5, 2.5);
\draw[->, line width=2mm] (15.5, -3.25) -- (16.5, -2.5);


% ------------- out --------------------------
\coordinate (base2) at ($(base1) + (24, 0)$);

\coordinate (l11) at (base2);
\node[rednode] at ( $(l11) + (0, 0)$) (greennode1) {};
\node[greennode] at ( $(l11) + (-1.5, -1)$) (greennode2) {};
\node[rednode] at ( $(l11) + (1, 1.5)$) (rednode1) {};
\node[greennode] at ( $(l11) + (-0.75, 1.75)$) (rednode2) {};
\node[rednode] at ( $(l11) + (1, -1.3)$) (orangenode1) {};
\node[bluenode] at ( $(l11) + (2, .5)$) (bluenode1) {};
\node[orangenode] at ( $(l11) + (2.75, -0.6)$) (bluenode2) {};
\node[orangenode] at ( $(l11) + (3.25, 1.75)$) (bluenode3) {};
\draw[very thick] (greennode2) -- (orangenode1);
\draw[very thick] (greennode2) -- (rednode2);
\draw[very thick] (rednode1) -- (rednode2);
\draw[very thick] (rednode2) -- (greennode1);
\draw[very thick] (greennode1) -- (greennode2);
\draw[very thick] (greennode1) -- (orangenode1);
\draw[very thick] (greennode1) -- (bluenode1);
\draw[very thick] (rednode1) -- (bluenode1);
\draw[very thick] (bluenode1) -- (bluenode2);
\draw[very thick] (bluenode1) -- (bluenode3);
\draw[very thick] (orangenode1) -- (bluenode1);


% \draw[->, very thick] (-2, 0) -- (-1, 0);
% \draw[->, very thick] (-2, -3) -- (-1.5, -4);
% \draw[->, very thick] (-2, 3) -- (-1.5, 4);


\end{tikzpicture}
% }

==> includes/graph_observation.tex <==
\begin{tikzpicture}
	\addLayer{\scene}{cscene}{};
	\addImage{\scene}{./includes/Render.png};
	\addImage{\layertwo}{./includes/Wire.png};
	\addImage{\layerthree}{./includes/Arch.png};




	\begin{scope}
		\myGlobalTransformation{0}{\layertwo};
		\node (l2n1a) at (0.9,3.6) [style=node2] {};
		\node (l2n2a) at (0.4,3.0) [style=node2] {};

		\node (l2n3a) at (2.9,2.4) [style=node2] {};
		\node (l2n4a) at (3.4,1.4) [style=node2] {};

		\node (l2n5a) at (1.6,1.2) [style=node2] {};
		\node (l2n6a) at (2.1,1.2) [style=node2] {};
		\node (l2n8a) at (2.7,0.9) [style=node2] {};

		\node (l2n7a) at (2.1,2.4) [style=node2] {};

		\node (l2n1b) at (0.7,3.6) [style=node2] {};
		\node (l2n2b) at (1.1,3.3) [style=node2] {};

		\node (l2n3b) at (3.3,2.5) [style=node2] {};
		\node (l2n4b) at (3.7,1.3) [style=node2] {};

		\node (l2n5b) at (1.3,1.1) [style=node2] {};
		\node (l2n6b) at (2.3,1.5) [style=node2] {};
		\node (l2n8b) at (2.5,0.9) [style=node2] {};

		\node (l2n7b) at (2.1,2.6) [style=node2] {};
	\end{scope}

	\begin{scope}
		\myGlobalTransformation{0}{\layerthree};
		\node (l3n1) at (1.2,3.5) [style=node3] {};
		\node (l3n2) at (0.7,3.2) [style=node3] {};

		\node (l3n3) at (3.0,2.4) [style=node3] {};
		\node (l3n4) at (3.4,1.5) [style=node3] {};

		\node (l3n5) at (1.5,1.2) [style=node3] {};
		\node (l3n6) at (2,1.2) [style=node3] {};
		\node (l3n8) at (2.8,0.8) [style=node3] {};

		\node (l3n7) at (2,2.4) [style=node3] {};
	\end{scope}

	\addAgentLayer{\layeragent}{cagent}{Actions}{2.8}{1.5};

	\begin{scope} [cm={1,0,\cma,\cmb,(0,\layeragent)}]
		\node [circle, minimum size=\layerwidth/3, cm={1,0,\cma,\cmb,(0,0)}] at (2.8,1.5) (c) {};
		\node (lan1) at (c.0) [style=nodeagent] {};
		\node (lan2) at (c.60) [style=nodeagent] {};
		\node (lan3) at (c.120) [style=nodeagent] {};
		\node (lan4) at (c.180) [style=nodeagent] {};
		\node (lan5) at (c.240) [style=nodeagent] {};
		\node (lan6) at (c.300) [style=nodeagent] {};
	\end{scope}


	\begin{scope}
		\myGlobalTransformation{0}{\layerfour};
		\node (l4n1) at (1,3.5) [style=node4] {};
		\node (l4n2) at (3.4,2.4) [style=node4] {};
		\node (l4n3) at (2,1.2) [style=node4] {};
	\end{scope}

	\draw[style=inter] (l2n1a) -- (l3n1);
	\draw[style=inter] (l2n2a) -- (l3n2);
	\draw[style=inter] (l2n3a) -- (l3n3);
	\draw[style=inter] (l2n4a) -- (l3n4);
	\draw[style=inter] (l2n5a) -- (l3n5);
	\draw[style=inter] (l2n6a) -- (l3n6);
	\draw[style=inter] (l2n7a) -- (l3n7);
	\draw[style=inter] (l2n8a) -- (l3n8);

	\draw[style=inter] (l2n1b) -- (l3n1);
	\draw[style=inter] (l2n2b) -- (l3n2);
	\draw[style=inter] (l2n3b) -- (l3n3);
	\draw[style=inter] (l2n4b) -- (l3n4);
	\draw[style=inter] (l2n5b) -- (l3n5);
	\draw[style=inter] (l2n6b) -- (l3n6);
	\draw[style=inter] (l2n7b) -- (l3n7);
	\draw[style=inter] (l2n8b) -- (l3n8);


	\draw[style=same, color=c3] (l3n1) -- (l3n2);
	\draw[style=same, color=c3] (l3n7) -- (l3n2);
	\draw[style=same, color=c3] (l3n7) -- (l3n1);
	\draw[style=same, color=c3] (l3n7) -- (l3n3);
	\draw[style=same, color=c3] (l3n4) -- (l3n5);
	\draw[style=same, color=c3] (l3n5) -- (l3n6);
	\draw[style=same, color=c3] (l3n8) -- (l3n6);
	\draw[style=same, color=c3] (l3n8) -- (l3n4);

	\draw[style=inter] (l3n1) -- (l4n1);
	\draw[style=inter] (l3n2) -- (l4n1);

	\draw[style=inter] (l3n3) -- (l4n2);
	\draw[style=inter] (l3n4) -- (l4n2);

	\draw[style=inter] (l3n5) -- (l4n3);
	\draw[style=inter] (l3n6) -- (l4n3);
	\draw[style=inter] (l3n8) -- (l4n3);


	\draw[style=highlight] (lan6) -- (l3n8);
	\draw[style=highlight] (lan6) -- (l3n4);
	\draw[style=highlight] (lan1) -- (l3n4);
	\draw[style=highlight] (lan5) -- (l3n6);

	\draw[style=highlight] (l2n4a) -- (lan6);
	\draw[style=highlight] (l2n4a) -- (lan1);
	\draw[style=highlight] (l2n6a) -- (lan5);
	\draw[style=highlight] (l2n8a) -- (lan6);

	\draw[style=highlight] (l2n4b) -- (lan1);
	\draw[style=highlight] (l2n6b) -- (lan5);

	\addLayer{\layertwo}{c2}{Objects};
	\addLayer{\layerthree}{c3}{Places};
	\addLayer{\layerfour}{c4}{Rooms};

\end{tikzpicture}


==> includes/overview_figure_diamond.tex <==

% \resizebox{240pt}{175pt}{%
\begin{tikzpicture}
    \node at (0, 0) (dsg) {
        \begin{minipage}{\columnwidth}
            \centering
            \includegraphics[width=0.9\columnwidth, trim=0 110 450 0, clip]{DSG_with_layer_labels.png}
            \caption*{\Large{(a) DSG incrementally constructed}}
        \end{minipage}
   };
    \node at (8, -6) (obs){
        \begin{minipage}{\columnwidth}
            \centering
            \vspace{6mm}
            \resizebox{0.8\columnwidth}{!}{\input{./includes/graph_observation.tex}}
            \vspace{4mm}
            \caption*{\Large{(b) Observations derived}}
        \end{minipage}
    };
    \node at (0, -10) (gnn) {
        \begin{minipage}{\columnwidth}
            \centering
            \reflectbox{\resizebox{0.6\columnwidth}{!}{\input{./includes/gnn_figure.tex}}}
            \vspace{5mm}
            \caption*{\Large{(c) GNN policy navigates}}
        \end{minipage}

    };
    \node at (-8, -6) (robot) {
        \begin{minipage}{\columnwidth}
            \centering
            \includegraphics[width=0.7\columnwidth, trim=350 0 350 150, clip]{./includes/racecar_3pv}
            \caption*{\Large{(d) Robot executes trajectory}}
        \end{minipage}
     };

    \draw[->, very thick] ($(dsg.east) + (0, 0.5)$) -| ($(obs.north) + (0, 1)$);
    \draw[->, very thick] ($(obs.south) + (0, -0)$) |- ($(gnn.east) + (0, -1)$);
    \draw[->, very thick] ($(gnn.west) + (0, -1)$) -| (robot.south);
    \draw[->, very thick] ($(robot.north) + (0, 1)$) |- ($(dsg.west) + (-1, 0)$);

\end{tikzpicture}
% }


==> sections/discussion.tex <==
%!TEX root = ../main.tex

\section{Discussion: Queries and Opportunities} %Limitations}
\label{sec:discussion}



==> sections/distribution-statement.tex <==

\blfootnote{
    DISTRIBUTION STATEMENT A. Approved for public release. Distribution is unlimited.\\
    This material is based upon work supported by the Under Secretary of Defense for Research and Engineering under Air Force Contract No. FA8702-15-D-0001. Any opinions, findings, conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the Under Secretary of Defense for Research and Engineering.
  }


==> sections/usepackages.tex <==
% !TeX root = ../main.tex
% \usepackage{mathtools}
% % to use subfigure
% % \usepackage{subcaption} Breaks arxiv submission...
% \usepackage{graphicx}
% \graphicspath{{img/}}
% % To import svg, and automatic workflow with inkscape.
% % But including svg also includes subfig which seems to collide with subfigure
% % This gives the error main.tex|143 error| Undefined control sequence. \sf@counterlist
% % Just remove deprecated subfigure, and use subcaptions instead...
% % !! WARNING requires installation of inkscape !!
% \usepackage[svgpath=img]{svg}
% % To import eps
% % WARNING: make sure that:
% % 1) sudo apt-get install texlive-font-utils #https://tex.stackexchange.com/a/231225
% % 2) you use -shell-escape in your compiler line
% \usepackage{epstopdf}
% % This must coincide with the path of graphicx to work!
% \epstopdfsetup{outdir=./img/}
% % To import pgf figures.
% \usepackage{pgf}
% % To use svgscale before calling input on a pdf_tex file or svg
% \usepackage{calc}
% To solve the issue of relative paths inside pgf.
\newcommand\inputpgf[2]{{
\let\pgfimageWithoutPath\pgfimage
\renewcommand{\pgfimage}[2][]{\pgfimageWithoutPath[##1]{#1/##2}}
\input{#1/#2}
}}

% For fancy todo notes.
% \usepackage{todonotes}
% For hyphenation, underlining, striking...
% \usepackage{soul}
% % To solve a bug with titlesec, and with makeidx
% \usepackage{etoolbox}
% % To get math functionality
% \usepackage{amsmath}
% % Use amsmath to create my own definition equality symbol
% \newcommand\defeq{\mathrel{\overset{\makebox[0pt]{\mbox{\tiny def}}}{=}}}
% % For nice math symbols
% \usepackage{amssymb}
% % Better than \boldsymbol, use \bm
% \usepackage{bm}
% % http://ctan.org/pkg/adjustbox
% \usepackage[export]{adjustbox}
% To add tables with even width
\usepackage{tabularx}
\newcolumntype{Y}{>{\centering\arraybackslash}X} % To make columns content centered
% To draw
% \usepackage{tikz}
% % To draw factor graphs in latex.
% \usetikzlibrary{bayesnet}
% % Set variables for factor graph distances.
% \newlength{\state} % Edge distance btw states
% \setlength{\state}{1cm}
% % For URLs
% \usepackage{url}
% % For mulicolumn
% \usepackage{array}
% % For copyright letters
% \usepackage{textcomp}
% % To avoid commands ignoring space after
% \usepackage{xspace}
% % To do nice minimalistic tables
% % and better spacing above and below the various rules in the table
% \usepackage{booktabs}
% % To have footnotes in tables
% % \usepackage{tablefootnote}
% % To allow for letters in enumerate (i, ii, ...)
% %\usepackage[shortlabels]{enumitem}
% % For citations to be ordered
% \usepackage{cite}
% % For multi rows in tables
% \usepackage{multirow}
% % To allow breaking lines inside tables
% \usepackage{makecell}
% % To avoid clash btw IEEE and enumitem, concerning double definition of labelindent
% % labelindent command exists for legacy reasons in the IEEE template, disable it:
% \let\labelindent\relax
% \usepackage{enumitem}
% \setlist[itemize]{leftmargin=*}
% % \setlist[enumerate]{wide = 0pt, leftmargin=*}
% % To have named colors.
% \usepackage{comment}
% \usepackage{color}

% % \newcommand{\blue}[1]{{\color{blue}#1}}
% % \newcommand{\green}[1]{{\color{green}#1}}
% % \newcommand{\red}[1]{{\color{red}#1}}
% \newcommand{\orange}[1]{{\color{orange}#1}}
% % Useful colored comments
% \newcommand{\Rebuttal}[1]{\blue{#1}}
% \newcommand{\TR}[1]{\orange{{\bf TR:}~#1}\\}
% % \newcommand{\LC}[1]{\red{{\bf LC:}~#1}}
% \newcommand{\TODO}[1]{
% \orange{{\bf TODO:}~#1} % Comment this line to remove TODOs
% }
% % Hyperref must be set last.
% % For links
% \usepackage{hyperref}
% \hypersetup{
%     colorlinks,
%     linkcolor={red!50!black},
%     citecolor={blue!50!black},
%     urlcolor={blue!80!black}
% }
% % Cleverer referencing
% % Hyperref must be set before cleveref or cref won't work
% \usepackage[capitalize]{cleveref}
% \usepackage{xspace}
% \renewcommand{\Cref}[1]{\cref{#1}} % Hack to make everything abbreviated.
% %\crefformat{section}{\S#2#1#3} % Change section word for symbol
% %\crefformat{subsection}{\S#2#1#3}
% %\crefformat{subsubsection}{\S#2#1#3}
% % Increase secnumdepth to also be able to reference paragraphs
% \setcounter{secnumdepth}{6}

\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

